Learning Object Permanence from Videos via Latent Imaginations

While human infants exhibit knowledge about object permanence from two months of age onwards, deep-learning approaches still largely fail to recognize objects' continued existence. We introduce a slot-based autoregressive deep learning system, the looped location and identity tracking model Loci-Looped, which learns to adaptively fuse latent imaginations with pixel-space observations into consistent latent object-specific what and where encodings over time. The novel loop empowers Loci-Looped to learn the physical concepts of object permanence, directional inertia, and object solidity through observation alone. As a result, Loci-Looped tracks objects through occlusions, anticipates their reappearance, and shows signs of surprise and internal revisions when observing implausible object behavior. Notably, Loci-Looped outperforms state-of-the-art baseline models in handling object occlusions and temporary sensory interruptions while exhibiting more compositional, interpretable internal activity patterns. Our work thus introduces the first self-supervised interpretable learning model that learns about object permanence directly from video data without supervision.

==> algorithm.tex <==
%\clearpage

\section{Loci-Looped Algorithm \protect\footnote{Reproduced from \cite{traub_learning_2023}} }
\label{app:pseudocode}
In the remainder, we denote scalar values by lower-case letters, tensors by upper-case letters, and vectors by bold letters. Moreover, we denote slot-specific activities with a subscript $k\in {1,..,K}$ and time by the superscript $t$. We drop $t$ for temporary values.

%We now first define data and neural encoding sizes and types used throughout Loci's processing pipeline.  We then specify neural activity initialization. Finally, we detail the unfolding overall processing loop.

\subsection{Slot-wise encoder}
\paragraph{Inputs} The encoder inputs at each time step $t$ consist of: 
\begin{itemize}
    \item RGB input image $I^t \in \mathbb{R}^{H\times W\times 3}$,
    \item MSE map $E^t \in \mathbb{R}^{H\times W\times 1}$ (pixel-wise mean squared error between $I^t$ and $\hat{R}^t$),
    \item Slot-specific RGB image reconstructions $\hat{R}^t_k \in \mathbb{R}^{H\times W\times 3}$,
    \item Slot-specific visibility mask predictions $\hat{M}^{t,v}_k \in \mathbb{R}^{H\times W\times 1}$,
    \item Slot-specific visibility mask complements $\hat{M}^{t,s}_k=\sum_{k' \in \{1,..,K\}\setminus k} \hat{M}^{t,v}_{k'}$
    \item Slot-specific object mask predictions $\hat{M}^{t,o}_k \in \mathbb{R}^{H\times W\times 1}$,
    \item Slot-specific isotropic Gaussian position map predictions $\hat{Q}^t_k \in \mathbb{R}^{H\times W}$,
    \item Background mask $\hat{M}^t_{bg} \in \mathbb{R}^{H\times W}$, which is equivalent to $1-\sum_{k \in \{1,..,K\}} \hat{M}^t_{k}$
\end{itemize}

\paragraph{Outputs} Based on these inputs, the slot-wise encoder network generates latent codes:
\begin{itemize}    
    \item Slot-specific Gestalt codes $\tilde{G}^t_k \in \mathbb{R}^{D_g}$,
    \item Slot-specific position codes $\tilde{P}^t_k \in \mathbb{R}^4$ encode an isotropic Gaussian $(\boldsymbol{\mu}^t_k,\sigma^t_k)$ and a slot-priority code $z^t_k$,
\end{itemize}
where $D_g$ denotes the size of the Gestalt code and $\boldsymbol{\mu}^t_k \in \mathbb{R}^2$.

\subsection{Slot-wise decoder - reconstruction}
\paragraph{Inputs} The outputs of all slots from the encoding module $\tilde{P}^{t}$ and $\tilde{G}^{t}$ then act as the input to the decoder.
\paragraph{Outputs} The output of the decoder includes the slot-respective masks and RGB reconstructions: 
\begin{itemize}
    \item Slot-specific visibility mask outputs $\tilde{M}^{t, v}_k \in \mathbb{R}^{H\times W}$,
    \item Slot-specific object mask outputs $\tilde{M}^{t,o}_k \in \mathbb{R}^{H\times W}$,
    \item Slot-specific RGB image reconstructions $\tilde{R}^{t}_k \in \mathbb{R}^{H\times W\times 3}$,
\end{itemize}
Further, we compute the slot-specific occlusion state $\tilde{O}^t_k$ as a function of $\tilde{M}^{t, v}_k$ and $\tilde{M}^{t, o}_k$, as specified in Equation~\ref{eq:occlusionstate}. We generate the combined reconstructed image $\hat{R}^{t}$ by summing all slot reconstructions $\tilde{R}^{t}_k$ and the background estimate $\tilde{R}_{bg}$ weighted with their corresponding masks $\tilde{M}^{t}_k$ and $\tilde{M}^{t}_{bg}$, as specified further in Algorithm~\ref{algo:loci}. The reconstructed image $\hat{R}^{t}$ is subject to the reconstruction loss (see Equation~\ref{eq:reconstructionloss}) and the occlusion state $\tilde{O}^t_k$ serves as input to the update gate controller. 

\subsection{Update module}
The slot-wise update module consists of an update gate controller and an update gate. The update gate controller takes the inputs,
\begin{itemize}    
    \item Slot-specific encoder Gestalt codes $\tilde{G}^t_k \in \mathbb{R}^{D_g}$,
    \item Slot-specific encoder position codes $\tilde{P}^t_k \in \mathbb{R}^4$,
    \item Slot-specific encoder occlusion state $\tilde{O}^t_k \in \mathbb{R}^{D_g}$,
    \item Slot-specific predicted Gestalt codes $\hat{G}^t_k \in \mathbb{R}^{D_g}$,
    \item Slot-specific predicted position codes $\hat{P}^t_k \in \mathbb{R}^4$,
    \item Slot-specific predicted occlusion state $\hat{O}^t_k \in \mathbb{R}^{D_g}$,
    \item Slot-specific previous position codes $P^{t-1}_k \in \mathbb{R}^4$
\end{itemize}

and outputs gate activation:
\begin{itemize}    
    \item Slot-specific Gestalt gate activation $\alpha^{t,G}_k \in [0,1)$,
    \item Slot-specific position gate activation $\alpha^{t,P}_k \in [0,1)$.
\end{itemize}

The update gate then linearly interpolates between $\tilde{G}^t_k$ and $\hat{G}^t_k$, as well as $\tilde{P}^t_k$ and $\hat{P}^t_k$, where a higher activation opens the gate and gives more weighting to $\tilde{G}^t_k$ or $\tilde{P}^t_k$. Finally, the update module produces:
\begin{itemize}    
    \item Slot-specific Gestalt codes $G^t_k \in \mathbb{R}^{D_g}$,
    \item Slot-specific position codes $P^t_k \in \mathbb{R}^4$,
\end{itemize}

\subsection{Transition module}
A transition module is used to process interaction dynamics within and between these slot-respective codes and creates a prediction for the next state, which is fed into the decoder.
The input to the transition module equals $G_k^t$, $P_k^t$, $\alpha^{t,G}_k$ and $\alpha^{t,P}_k$.
It is processed across slots and per slot in the respective layers:
Multi-Head Attention predicts slot interactions (across slots), while
GateL0RD predicts slot-specific dynamics (per slot).
We use two attention layers with ten heads each with GateL0RD layers in between.

\paragraph{Outputs} The outputs of the transition module $\hat{G}^{t+1}_k$ and $\hat{P}^{t+1}_k$ have the same size as $G^t_k$ and $P^t_k$. Additionally, recurrent, slot-respective hidden states $\hat{H}^t_k$ are maintained in the time-recurrent GateL0RD layers:
\begin{itemize}    
    \item Slot-specific position codes $\hat{P}^{t+1}_k \in \mathbb{R}^4$,
    \item Slot-specific Gestalt codes $\hat{G}^{t+1}_k \in \mathbb{R}^{D_g}$,
    \item Slot-specific GateL0RD-layer-respective hidden states $\hat{H}^t_k \in \mathbb{R}^{D_h}$,
\end{itemize}
where $D_h$ denotes the size of the recurrent latent states.

\subsection{Slot-wise decoder - prediction}
\paragraph{Inputs} The outputs of all slots from the transition module $\hat{P}^{t+1}$ and $\hat{G}^{t+1}$ then act as the input to the decoder.
\paragraph{Outputs} The output of the decoder includes the slot-respective masks and RGB reconstructions: 
\begin{itemize}
    \item Slot-specific visibility mask outputs $\hat{M}^{t+1, v}_k \in \mathbb{R}^{H\times W}$,
    \item Slot-specific object mask outputs $\hat{M}^{t+1,o}_k \in \mathbb{R}^{H\times W}$,
    \item Slot-specific RGB image reconstructions $\hat{R}^{t+1}_k \in \mathbb{R}^{H\times W\times 3}$,
\end{itemize}
which are then used as part of the input at the next iteration as specified above. Further, we compute the slot-specific occlusion state $\hat{O}^t_k$ as a function of $\hat{M}^{t+1, v}_k$ and $\hat{M}^{t+1, o}_k$, as specified in \ref{eq:occlusionstate}.

We generate the combined reconstructed image $\hat{R}^{t+1}$ by summing all slot estimates $\hat{R}^{t+1}_k$ and the background estimate $\hat{R}_{bg}$ weighted with their corresponding masks $\hat{M}^{t+1}_k$ and $\hat{M}^{t+1}_{bg}$, as specified further in Algorithm~\ref{algo:loci}. The predicted image $\hat{R}^{t+1}$ is subject to the prediction loss (see \ref{eq:reconstructionloss}) and the occlusion state $\tilde{O}^{t+1}_k$ serves as input to the update gate controller in the next timestep.


\begin{algorithm}[b!]
   \caption{\texttt{Loci-v2-Algorithm} (main processing loop)}
   \label{algo:loci}
\begin{algorithmic}[1]
    \vspace{.1cm}
    \STATE \textbf{Inputs:} Input video $I \in \mathbb{R}^{T \times H \times W \times 3}$, static background $\hat{R}_{bg} \in \mathbb{R}^{H \times W \times 3}$
    \STATE \textbf{Network parameters:} $\Theta_{encoder}$, $\Theta_{update}$, $\Theta_{transition}$, $\Theta_{decoder}$
    \STATE \textbf{Additional parameters:} 
    initialization parameters $\Theta_{init}$; background threshold $\theta_{bg}$, which is encoded as a uniform offset mask $\Tilde{M}_{bg} \leftarrow \theta_{bg}$; number of slots $K$; processing steps $T$
    \\\vspace{-.1cm}
    \hrulefill
    \\\vspace{.1cm}
    \STATE  Initialize $H_k^{1}, \hat{R}^{1}_k, \hat{R}^{1}, \hat{M}^{1,o}_k, \hat{M}^{1,v}_k, \hat{Q}^{1}_k$ %\COMMENT{see Section~\ref{sec:algini} for details}
    %\vspace{-.3cm}
    \FOR{$t=1\dots T $}
            \vspace{.1cm}
        \STATE \COMMENT{\underline{Pre-processing:}}
%            \vspace{-.3cm}
        \STATE $E^t \leftarrow \sqrt{\texttt{Mean}\left(\left(I^t - R_{bg}\right)^2, axis=\text{'rgb'}\right)}\circ \sqrt[4]{\texttt{Mean}\left(\left(I^{t} - \hat{R}^{t}\right)^2, axis=\text{'rgb'}\right)}$
        \STATE \texttt{compute complement} $\hat{M}^{t,s}_k$
            \vspace{.1cm}
        \STATE \COMMENT{\underline{Slot-wise encoder:}}
%            \vspace{-.3cm}
%        \FOR {$k\in K$}
            \STATE $S^t_k \leftarrow Encoder_{Trunk}(I^t, E^t, \hat{R}^t_k, \hat{M}^{t,v}_{k}, \hat{M}^{t,o}_{k}, \hat{M}^{t,s}_{k}, \hat{Q}^t_k, \hat{M}_{bg}^t)$
            %\STATE\COMMENT{Slot Gestalt G}
            \STATE $\tilde{G}^t_k \leftarrow Encoder_{Gestalt}(S^t_k)$
            %\STATE\COMMENT{Slot Position P}
            \STATE $P'^t_k \leftarrow Encoder_{Position}(S^t_k)$
            \STATE $\tilde{P}^t_k \leftarrow \texttt{concat}\left[\boldsymbol{\mu}^t_k, \sigma^t_k, z^t_k\right] \leftarrow \texttt{concat} \left[Encoder_{\boldsymbol{\mu}}(P'^t_k), Encoder_{\boldsymbol{\sigma}}(P'^t_k), Encoder_{z}(P'^t_k)\right]$
 %       \ENDFOR

        \vspace{.1cm}   
       \STATE\COMMENT{\underline{Slot-wise decoder - reconstruction (see decoder - prediction and post-processing):}}
       
       \STATE $\tilde{O}^{t}_k \leftarrow 1- \frac{\sum_{i,j} [\tilde{M}^{t,v}_k(i,j) > \theta_{bg}]}{\sum_{i,j} [\tilde{M}^{t,o}_k(i,j) > \theta_{bg}] + 0.0001}$

       \STATE $\tilde{R}^{t} \leftarrow \texttt{sum}(\texttt{concat}\left[\tilde{R}^{t}_1,..,\tilde{R}^{t}_K,\tilde{R}_{bg}\right]\circ \tilde{M}^{t,v}, axis=\text{'K'})$
                           
        \vspace{.1cm}
        \STATE \COMMENT{\underline{Update module:}}
           \STATE $[\alpha^{t,G}_k, \alpha^{t,P}_k] \leftarrow UpdateController(\tilde{P}^t_k, \tilde{G}^t_k, \tilde{O}^t_k, \hat{P}^t_k, \hat{G}^t_k,\hat{O}^t_k, P^{t-1}_k)$  
           \STATE $G^t_k \leftarrow \alpha^{t,G}_k \tilde{G}^t_k + (1- \alpha^{t,G}_k)  \hat{G}^t_k$ 
           \STATE $P^t_k \leftarrow \alpha^{t,P}_k \tilde{P}^t_k + (1- \alpha^{t,P}_k) \hat{P}^t_k$     
 
            \vspace{.1cm}
        \STATE \COMMENT{\underline{Transition module:}}
%            \vspace{-.3cm}
%        \STATE\COMMENT{Multi-Head Attention processes slot interactions (over slots)}
%        \STATE\COMMENT{Gate-L0rd processes dynamics (per slot)}
        \STATE $\hat{G}^{t+1}, \hat{P}^{t+1}, H^{t+1} = TransitionModule(G^t, P^t, \alpha^{t,G}_k, \alpha^{t,P}_k, H^{t})$ 
            \vspace{.1cm}
        \STATE \COMMENT{\underline{Gestalt binarization:}}
        \STATE $\hat{G}^{t+1} \leftarrow \texttt{Sigmoid}(\hat{G}^{t+1})$ 
        \STATE $\hat{G}^{t+1} \leftarrow \hat{G}^{t+1} + \hat{G}^{t+1} (1 - \hat{G}^{t+1}) \mathcal{N}(0, 1)$
            \vspace{.1cm}
        \STATE\COMMENT{\label{algo:loci_decoder}\underline{Slot-wise decoder - prediction:}}
%            \vspace{-.3cm}
        \STATE \COMMENT{$p$ encodes all pixel positions normalized to $[-1,1]$, $\texttt{width}$ the number of pixels in a row}
%            \vspace{-.3cm}
            \STATE $\hat{Q}^{t+1}_k \leftarrow \exp \left(
            \frac{ - (p - \hat{\boldsymbol{\mu}}^{t+1}_k)^2}
            { 2 \max \left(\frac{1}{\texttt{width}}, \hat{\sigma}^{t+1}_k \right)^2}
            \right)$ 
            %\vspace{-.2cm}
            \STATE $decode_k \leftarrow \texttt{Priority-Based-Attention}(\hat{G}^{t+1}_k, \hat{Q}^{t+1}_k, \hat{\mathbf{z}}^{t+1})$
            \STATE $\hat{R}^{t+1}_k, \Tilde{M}^{t+1}_k \leftarrow Decoder_{Trunk}(decode_k)$
                \vspace{.1cm}
            \STATE \COMMENT{\underline{Post-processing:}}
%                \vspace{-.3cm}
            \STATE $[\hat{M}^{t+1,v}_1, \dots, \hat{M}^{t+1,v}_K, \hat{M}^{t+1}_{bg}] \leftarrow \texttt{softmax}(\texttt{concat}[\Tilde{M}^{t+1}_1, \dots, \Tilde{M}^{t+1}_K, \Tilde{M}_{bg}], axis=\text{'K'})$
            
            %\STATE $\hat{M}^{t+1,o}_k \leftarrow \texttt{softmax}(\texttt{concat}[\Tilde{M}^{t+1}_k, \Tilde{M}_{bg}], axis=\text{'K'})[0]$
            
            \STATE $\hat{M}^{t+1,o}_k \leftarrow \frac{\mathrm{exp}(\hat{M}^{t+1}_k)}{\mathrm{exp}(\hat{M}^{t+1}_k) + \mathrm{exp}(\hat{M}^{t+1}_{bg})},$
            
            \STATE $\hat{O}^{t+1}_k \leftarrow 1- \frac{\sum_{i,j} [\hat{M}^{t+1,v}_k(i,j) > \theta_{bg}]}{\sum_{i,j} [\hat{M}^{t+1,o}_k(i,j) > \theta_{bg}] + 0.0001}$
            
            \STATE $\hat{R}^{t+1} \leftarrow \texttt{sum}(\texttt{concat}\left[\hat{R}^{t+1}_1,..,\hat{R}^{t+1}_K,\hat{R}_{bg}\right]\circ \hat{M}^{t+1,v}, axis=\text{'K'})$
    \ENDFOR
\STATE \textbf{return} $[\hat{R}^1 \dots \hat{R}^T]$
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[t!]
   \caption{\texttt{Priority-based-Attention}}
   \label{algo:atten}
\begin{algorithmic}[1]
    \vspace{.1cm}
    \STATE \textbf{Inputs:} 
    Gestalt: $G_k\in\mathbb{R}^{1,D_{g}}$, 
    Gaussian 2d position: $Q_k\in\mathbb{R}^{H'\times W'\times 1}$,
    priority: $\boldsymbol{z}\in\mathbb{R}^{K}$
    \STATE \textbf{Additional parameters:} values of the learnable $\boldsymbol{\theta^w}\in\mathbb{R}^{K}$ are initially set to $25$, while  $\boldsymbol{\theta^b}\in\mathbb{R}^{K}=\{0, 1, \dots, (K - 1)\}$ induces a default slot-order bias.
    \\\vspace{-.1cm}
    \hrulefill
    \\\vspace{.1cm}
    \STATE $\boldsymbol{z'} \leftarrow (\boldsymbol{z} \cdot K + \mathcal{N}(0, 0.1) + \boldsymbol{\theta^b}) \circ \boldsymbol{\theta^w}$ \COMMENT{Scale priorities and add Noise}
    \STATE \COMMENT{Subtract Gaussian attention from other slots, scaled by priority ($\sigma$ denotes the sigmoid)}
    \STATE $Q'_k \leftarrow \max(0, Q_k - \sum_{k'\in \{1, \dots, K\}\setminus k} \sigma(z'_k - z'_{k'}) \cdot Q_i)$ 
    \STATE $combine_k \leftarrow Q'_k \times G_k$ \COMMENT{$combine_k\in\mathbb{R}^{H'\times W'\times D_{g}}$}
    \STATE \textbf{return} $combine_k$
\end{algorithmic}
\end{algorithm}



